Linear scaling computation of forces for the domain-decomposition linear Poisson--Boltzmann method

The Linearized Poisson--Boltzmann (LPB) equation is a popular and widely accepted model for accounting solvent effects in computational (bio-) chemistry. In the present article we derive the analytical forces of the domain-decomposition-based ddLPB-method with vdW or SAS surface. We present an efficient strategy to compute the forces and its implementation, allowing linear scaling of the method with respect to the number of atoms using the fast multipole method (FMM). Numerical tests illustrates the accuracy of the computation of the analytical forces and compares efficiency with other available methods.

==> introduction_Journal.tex <==
Most chemical processes and virtually all biochemical processes happen in condensed phase, a situation where the reacting part, or in general the studied part, is embedded in an environment which usually consists of a solvent. For this reason, solvation models, which take into account the effect of the environment on the interesting part (solute), are widely used in computational chemistry and biochemistry.
These models can be broadly divided into two classes, explicit solvation models and implicit (continuum) solvation models.
%Solvation models simulate the interaction between solute and solvent in computational chemistry \mn{and biochemistry}.
%In fact, the modeling of the solvation model can be broadly divided into two classes, explicit solvation models and implicit (continuum) solvation models. 
Explicit solvation models consider the molecular representation of both, the solute and solvent, making the method more accurate, but computationally expensive and also dependent on a large set of empirical parameters (force field).
%On the other hand, continuum solvation models treat the solvent as a continuum and only adopt the microscopic properties of the solute (with possibly a few solvent molecules). 
On the other hand, continuum solvation models treat the solvent as a continuum, described only by a few macroscopic properties. This approach, by its nature, cannot describe specific interactions and anisotropic environment, however it presents some large advantages, it reduces the computational cost significantly, requires fewer parameters and implicitly takes into account the sampling over the degrees of freedom of the solvent. For this reason, implicit solvation models are popular computational approaches to characterize solvent effects in the 
simulation of properties and processes of molecular systems in condensed phase \cite{TP94,HN95,RS99,CT99,OL00,TMC05}.

Some of the widely used continuum solvation models include the conductor-like screening model (COSMO), proposed in \cite{KS93}; the surface and simulation of volume polarization for electrostatics (SS(V)PE) \cite{Ch99, Ch06}; polarizable continuum model (PCM) \cite{TMC05, MST81, CMT97, BC98, CRSB03} to name a few. In this paper, we focus on the continuum solvation model based on the Poisson--Boltzmann (PB) equations \cite{YL90, NH91} which takes into account both the solvent relative dielectric permittivity and the ionic strength of the solvent.

We consider specifically the linearized Poisson--Boltzmann (LPB) equation which describes the electrostatic potential, $\psi$ of the solvation model in the following form
\begin{equation}\label{eq:lpb_equation}
-\nabla\cdot \left[ \varepsilon(\bx)\nabla \psi(\bx)\right]+\overline{\kappa}(\bx)^2\psi(\bx)=4\pi \rho_{\mathrm{M}}(\bx)\qquad \mathrm{in}\ \ \mathbb{R}^3,
\end{equation}
where $\varepsilon(\bx)$ is the space-dependent dielectric permittivity function, $\overline{\kappa}(\bx)$ is the modified Debye-H\"uckel parameter, and $\rho_{\mathrm{M}}(\bx)$ is the solute charge distribution.

We denote the solute cavity by $\Omega$ and the solvent region by $\Omega^{\mathrm{C}}=\mathbb{R}^3\setminus \Omega$. To describe the solute-solvent region we will use the van-der Waals (vdW) surface (see Fig.~\ref{fig:solute_cavity}). The solute cavity $\Omega$ is defined as a union of overlapping subdomains, $\Omega_j$, i.e.,
$$
\Omega=\bigcup_{j=1}^M \Omega_j,
\qquad 
\Omega_j=B_{r_j}(\bx_j),
$$
where each $\Omega_j$ is a vdW ball with radius $r_j$ and center $\bx_j$, and $M$ is the total number of atoms. Then $\varepsilon(\bx)$ has the form
\begin{equation*}
\varepsilon(\bx) = \begin{cases} 
        \varepsilon_1 & \mbox{ in } \Omega,\\
        \varepsilon_2  & \mbox{ in } \Omega^{\mathrm{C}},
      \end{cases}
\end{equation*}
where $\varepsilon_1$ and $\varepsilon_2$ are the solute and solvent's dielectric permittivity, respectively. Furthermore, $\overline{\kappa}(\bx)$ has the form
\begin{equation*}
\overline{\kappa}(\bx) = \begin{cases} 
        0 & \mbox{ in } \Omega,\\
        \sqrt{\varepsilon_2}\kappa  & \mbox{ in } \Omega^{\mathrm{C}},
      \end{cases}
\end{equation*}
where $\kappa>0$ is the Debye-H\"uckel screening constant of the solvent.

%\input{solute_cavity.tex}

\begin{figure}
    \centering
    \includegraphics[width=8cm]{h2co.pdf}
    \caption{Cavity example for a formaldehyde molecule}
    \label{fig:solute_cavity}
\end{figure}

The classical PCM and the COSMO model can be considered as the special cases for PB solvation models. In the classical PCM,  the solvent is represented as a polarizable continuous medium that is non-ionic ($\kappa =0$) whereas the COSMO is a reduced version of the PCM, where the solvent is represented as a conductor-like continuum. 

We would like to mention some of the widely used methods for solving the LPB equation such as the boundary element method (BEM), the finite difference method (FDM), and the finite element method (FEM), and we refer to \citenum{LZHM08} for a review. The main idea of the BEM is to recast the LPB equation as an integral equation defined on a two-dimensional solute-solvent interface \cite{YL90, BFZ02, ABWT09, BSR11}. It is an efficient way to solve the LPB equation, which can be optimized using fast multipole methods \cite{ZPH15} and the hierarchial treecode technique \cite{LZHM08}. The PAFMPB solver \cite{LCH10, ZPH15} uses the former optimization technique, whereas the TABI-PB \cite{WK13} uses the latter one. 
The PB-SAM solver developed by Head-Gordon et al. \cite{lotan2006analytical,yap2010new,yap2013calculating} discretizes the solute-solvent interface (such as the vdW surface) with grid points on atomic spheres like a collocation method and solves the associated linear system by use of the fast multipole method. It primarily targets the interaction of disjoint molecular compounds.
However, one of the limitations of all these solvers relying on integral equations and layer potentials is that it cannot be generalized to solve the nonlinear PB (NPB) equation as opposed to PDE-based methods such as the FDM or FEM.

The finite difference approach is the most popular method to solve linear or nonlinear PB equations. The main idea is to cover the region of interest with a big-box grid and choose different kinds of boundary conditions. Some of the popular software packages using the FDM include UHBD \cite{Madura95}, Delphi \cite{LiLi12}, MIBPB \cite{CCC10}, and APBS \cite{BSJ01, DCLN07, JE17}. One of the drawbacks of the FDM is that the cost can increase considerably with respect to the grid dimension.

The finite element approach, compared to FDM, provides more flexible mesh refinement and a proper convergence analysis \cite{CHX07}. The SDPBS and SMPBS offer fast and efficient approximations of the size-modified PB equation \cite{Xie14, YX15, JXYXY15, XYX17}.

In this paper, we focus on the domain decomposition (dd) framework. Recently, in \citenum{QSM19} a domain decomposition algorithm has been proposed for the LPB equation, which uses a particular Schwarz domain decomposition method to solve Eq.~\eqref{eq:lpb_equation}. The ideas of the ddLPB method can be traced back to the domain decomposition methods proposed for the COSMO model (ddCOSMO) \cite{CMS13, LSCMM13, LLSS14, LSLS14} and the PCM model (ddPCM) \cite{SCLM16, GLS17, NSSL19,
QSM18}. These methods do not require any mesh or grid of the molecular surface, are easy to implement, and about two orders of magnitude faster than the state of the art \cite{LLSS14}.
In particular, the ddCOSMO solver can perform up to thousands of times faster than equivalent existing algorithms.

Similar to the aforementioned dd approaches, the ddLPB method does also not require any mesh or grid but depends, as ddCOSMO and ddPCM, only on the Lebedev quadrature points \cite{LL99} on a two-dimensional sphere. Hence, it is conveniently applied to molecular dynamics without re-meshing the molecular surface as in the BEM. 
The ddLPB solver adopts a spectral Galerkin method for discretization and benefits from high sparsity of the involved matrices for the Laplace and screening Poisson equations in $\Omega$, which are coupled by a non-local integral equation on the boundary.
The latter takes the majority of cost but can be further accelerated using for example the fast multipole method (FMM).
Numerical implementations show that the ddLPB solver is very efficient even without acceleration techniques (see \citenum{QSM19} for details) and its FMM-acceleration is ongoing work in progress but not within the scope of this article. 
The focus of this work is to develop the framework of the computation of first derivatives and the forces for the ddLPB method, the FMM-acceleration is a subsequent step. As the spheres are centered around their nuclei, the computation of the forces becomes natural. By the nature of the problem, this is very technical task, but a necessity in order to make accessible the method to models requiring the gradient of the solvation energy with respect to the nuclear coordinates such as molecular dynamics or geometry optimization.



==> preamble_Journal.tex <==
\usepackage{chemformula} % Formula subscripts using \ch{}
\usepackage[T1]{fontenc} % Use modern font encodings
%% The amssymb package provides various useful mathematical symbols
\usepackage{amssymb}
%% The amsthm package provides extended theorem environments
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{subcaption}
\usepackage{color}
\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{calc,patterns}
%\pgfplotsset{compat=1.9}
%\pgfplotsset{compat=1.10}
% set up externalization
%flowchart
\usetikzlibrary{positioning} 
\usetikzlibrary{calc}
\usepackage{pgfplots}
\pgfplotsset{width=10cm,compat=1.9}
%For multirow
\usepackage{multirow}
%Sideway tabe
\usepackage{rotating}
%Scientific Notation number
\usepackage{siunitx}
\sisetup{round-mode=places,round-precision=4}
\pgfplotsset{every tick label/.append style={font=\large}}

%Reference package
\usepackage{hyperref}
\usepackage[all]{hypcap}

\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}
\newcommand{\black}{\color{black}}



==> tables.tex <==
\begin{table}
\centering
\begin{tabular}{|c | c  c c c  c | c c c c |}
\hline
\textbf{PDB} &   \multicolumn{5}{c |}{\textbf{ddLPB}} & \multicolumn{4}{c |}{\textbf{APBS}} \\
\textbf{Code}& & & & & & & & & \\ \hline
 & $\ell_{\max}$ & \textbf{Energy} & \textbf{Rel.} & \textbf{Mem.} & \textbf{Iter.} & $\boldsymbol{h}$ \textbf{(\AA)} & \textbf{Energy} & \textbf{Rel.} & \textbf{Mem.} \\
 & & \textbf{(kJ/mol)} & \textbf{En.} & \textbf{(GB)} & & &  \textbf{(kJ/mol)} & \textbf{En.} & \textbf{(GB)} \\
\hline\hline
\multirow{11}{*}{1ay3} & 2 & \num{-126.589131762828} & \num{0.0323164948306518} & \num{0.0347404479980469}  & 5 & \num{0.435333333333333} & \num{-134.712690246} & \num{0.0302325381455532} & \num{0.021484375} \\ \cline{2-10}
 & 3 & \num{-128.434697720959} & \num{0.0182084611431196} & \num{0.0462799072265625} & 6 & \num{0.0126995510295332} & \num{-134.0655697204} & \num{0.0252836011125421} & \num{0.0218124389648437}\\ \cline{2-10}
 & 4 & \num{-129.155354985977} & \num{0.0126995510295332} & \num{0.04156494140625} & 6 & \num{0.221333333333333} & \num{-132.6795806804} & \num{0.0146840725609733} & \num{0.0638046264648438}\\ \cline{2-10}
 & 5 & \num{-129.66071992107} & \num{0.00883639702120393} & \num{0.0473136901855469} & 6 & \num{0.169666666666667} & \num{-132.3780103358} & \num{0.0123777747580023} & \num{0.124382019042969}\\ \cline{2-10}
 & 6 & \num{-129.965314246586} & \num{0.00650799093716325} & \num{0.056884765625} & 6 & \num{0.133333333333333} & \num{-131.9790674549} & \num{0.00932680802269184} & \num{0.244762420654297}\\ \cline{2-10}
 & 7 & \num{-130.166818716427} & \num{0.00496763317526335} & \num{0.075164794921875} & 6 & \num{0.09} & \num{-131.5849477545} & \num{0.0063127271774888} & \num{0.790634155273438}\\ \cline{2-10}
($25$) & 8 & \num{-130.33081848577} & \num{0.00371397206364328} & \num{0.0921630859375} & 6 &  &  & &\\ \cline{2-10}
 & 9  & \num{-130.435556454953} & \num{0.00291332509077986} & \num{0.124881744384766} & 6 &  & & & \\ \cline{2-10}
 & 10  & \num{-130.546158773294} & \num{0.00206784935679195} & \num{0.152523040771484} & 6 &  & & &\\ \cline{2-10}
 & 12 & \num{-130.688605284043} & \num{0.000978947514262507} & \num{0.287326812744141} & 6 &  & & &\\ \cline{2-10}
 & fit & \num{-130.8166679} &  &  & & fit & \num{-130.7594987} & &\\ \hline
\multirow{11}{*}{1etn}& 2 & \num{-513.715822013828} & \num{0.0275382146640793} & \num{0.050567626953125}  & 5 & \num{0.464666666666667} & \num{-534.1625908574} & \num{0.0143886290577194} & \num{0.0651435852050781} \\ \cline{2-10}
 & 3 & \num{-519.2850994043839} & \num{0.0169955971269766} & \num{0.0740776062011719} & 6 & \num{0.407} & \num{-534.1284379231} & \num{0.0143237717487356} &  \num{0.0970687866210938}\\ \cline{2-10}
 & 4 & \num{-521.799384575673} & \num{0.0122360663869432} & \num{0.175880432128906} & 6 & \num{0.282} & \num{-531.2851154656} & \num{0.00892422857780166} &  \num{0.252143859863281}\\ \cline{2-10}
 & 5 & \num{-523.334044319146} & \num{0.0093309622611437} & \num{0.215728759765625} & 6 & \num{0.175666666666667} & \num{-529.5238800521} & \num{0.00557959679877631} &  \num{0.996250152587891}\\ \cline{2-10}
 & 6 & \num{-524.321642382571} & \num{0.0074614434828672} & \num{0.365215301513672} & 7 & \num{0.141666666666667} & \num{-529.0143511346} & \num{0.00461198815501399} & \num{1.82976150512695}\\ \cline{2-10}
 & 7 & \num{-525.133730860213} & \num{0.00592416357639553} & \num{0.598438262939453} & 7 & \num{0.0973333333333333} & \num{-528.2927463393} & \num{0.00324164191296269} &  \num{6.17082595825195}\\ \cline{2-10}
($180$)& 8 & \num{-525.753588853788} & \num{0.00475077512843282} & \num{0.903827667236328} & 7 &  &  & &\\ \cline{2-10}
 & 9 & \num{-526.291880418717} & \num{0.00373179157014931} & \num{1.36589050292969} & 7 &  &  & & \\ \cline{2-10}
 & 10 & \num{-526.696668383837} & \num{0.00296552973748861} & \num{1.91103363037109} & 7 &  &  & &\\ \cline{2-10}
 & 12 & \num{-527.224216980141} & \num{0.0019668825714307} & \num{3.64987945556641} & 8  &  &  & &\\ \cline{2-10}
 & fit & \num{-528.2632488} & &  & & fit & \num{-526.5857439} & &\\ \hline
 \multirow{11}{*}{1du9} & 2 & \num{-1193.27872719215} & \num{0.0412979620736239} & \num{0.071258544921875}  & 6 & \num{0.445} & \num{-1264.572354587} & \num{0.0206170750214751} & \num{0.211505889892578} \\ \cline{2-10}
 & 3 & \num{-1214.41307301635} & \num{0.0243182406135944} & \num{0.124252319335938} & 6 & \num{0.268} & \num{-1254.291831097} & \num{0.0123198211901749} &  \num{0.841773986816406}\\ \cline{2-10}
 & 4 & \num{-1224.29474579209} & \num{0.0163791232788578} & \num{0.235774993896484} & 6 & \num{0.183666666666667} & \num{-1249.622695918} & \num{0.00855143334586907} &  \num{2.61618041992187}\\ \cline{2-10}
 & 5 & \num{-1230.01840557186} & \num{0.0117806299258633} & \num{0.447315216064453} & 7 & \num{0.144} & \num{-1247.455043055} & \num{0.00680195375565648} &  \num{5.52729415893555}\\ \cline{2-10}
 & 6 & \num{-1233.55524842793} & \num{0.00893906543915} & \num{0.764183044433594} & 7 & \num{0.096} & \num{-1244.40978378} & \num{0.00434417140523682} & \num{20.456859588623}\\ \cline{2-10}
 & 7 & \num{-1236.22566064244} & \num{0.00679360723746203} & \num{1.21342468261719} & 7 & &  & &\\ \cline{2-10}
($380$)& 8 & \num{-1238.2298355528} & \num{0.00518341631799075} & \num{1.86652374267578} & 8 & & & &\\ \cline{2-10}
 & 9 & \num{-1239.6524365911} & \num{0.00404047252498142} &  \num{2.81149291992187} & 8 & & & &\\ \cline{2-10}
 & 10 & \num{-1240.8052928982} & \num{0.00311424660150949} & \num{4.0201530456543} & 8 & & & &\\ \cline{2-10}
 & 12 & \num{-1242.37826560882} & \num{0.0018504914461466} & \num{7.70277404785156} & 8 & & & &\\ \cline{2-10}
 & fit & \num{-1244.681538} & &  & &  fit & \num{-1239.027237} & &  \\ \hline
\end{tabular}
\caption{Solvation energy, memory, and number of iterations for ddLPB and APBS. ``Rel. En.'' stands for the relative error in the energy,  "Mem." stands for the memory,  ``Iter.'' stands for the number of macro-iterations,  and ``$h$'' stands for the grid spacing (APBS).}
\label{tab:sol_energy_1}
\end{table}

\begin{table}
\centering
\begin{tabular}{|c | c c c c c | c c c c|}
\hline
\textbf{PDB} &  \multicolumn{5}{c |}{\textbf{ddLPB}} & \multicolumn{4}{c |}{\textbf{APBS}} \\
\textbf{Code}&  & & & & & & & & \\ \hline
 & $\ell_{\max}$ & \textbf{Energy} & \textbf{Rel.} & \textbf{Mem.} & \textbf{Iter. } & $\boldsymbol{h}$ \textbf{(\AA)} & \textbf{Energy} & \textbf{Rel.} & \textbf{Mem.} \\
 & & \textbf{(kJ/mol)} & \textbf{En.} & \textbf{(GB)} & &  &  \textbf{(kJ/mol)} & \textbf{En.} &  \textbf{(GB)} \\
\hline\hline
\multirow{11}{*}{1gzz} & 2 & \num{-1519.23538570063} & \num{0.0475951072386028} & \num{0.145637512207031}  & 6 & \num{0.537666666666667} & \num{-1628.943660159} & \num{0.0271657622903853} & \num{0.367588043212891} \\ \cline{2-10}
 & 3 & \num{-1549.80661052458} & \num{0.0284300822700651} & \num{0.307849884033203} & 7 & \num{0.421333333333333} & \num{-1617.35320366} & \num{0.0198571485081708} &  \num{0.704723358154297}\\ \cline{2-10}
 & 4 & \num{-1564.64692350627} & \num{0.0191267268934696} & \num{0.634464263916016} & 7 & \num{0.282} & \num{-1607.443492112} & \num{0.0136083649159344} &  \num{2.27139282226562}\\ \cline{2-10}
 & 5 & \num{-1572.89423464632} & \num{0.0139565080084699} & \num{1.20589447021484} & 8 & \num{0.191} & \num{-1601.129745896} & \num{0.00962709527261677} &  \num{7.58325958251953}\\ \cline{2-10}
 & 6 & \num{-1578.06557749057} & \num{0.0107146060139749} & \num{2.12812805175781} & 8 & \num{0.144666666666667} & \num{-1597.545960845} & \num{0.00736726186411452} &  \num{18.8806800842285}\\ \cline{2-10}
 & 7 & \num{-1582.1489102292} & \num{0.00815477485440078} & \num{3.52715301513672} & 8  &  & & & \\ \cline{2-10}
 ($940$)& 8 & \num{-1585.2220877375} & \num{0.00622820750165356} & \num{5.53937149047852} & 8 &  & & &\\ \cline{2-10}
 & 9  & \num{-1587.36784820018} & \num{0.00488303559308325} & \num{8.34081268310547} & 8 &  & & &\\ \cline{2-10}
 & 10  & \num{-1589.11640012914} & \num{0.00378687272848493} & \num{12.0966720581055} & 8 &  & & &\\ \cline{2-10}
 & 12 & \num{-1591.39680998403} & \num{0.00235728945011961} & \num{23.3187599182129} & 8 &  & & &\\ \cline{2-10}
 & fit & \num{-1595.157057} & &  & & fit & \num{-1585.862497} & &\\ \hline
\multirow{11}{*}{1jvu} & 2 & \num{-6273.88446560369} & \num{0.0401727835274069} & \num{0.536357879638672}  & 6 & \num{0.548} & \num{-6635.431676832} & \num{0.018662525664579} & \num{1.24731063842773} \\ \cline{2-10}
 & 3 & \num{-6381.72307611824} & \num{0.0236748014676603} & \num{1.3232536315918} & 8 & \num{0.445} & \num{-6619.209075601} & \num{0.01617205379362} &  \num{2.28483581542969}\\ \cline{2-10}
 & 4 & \num{-6438.820145177563} & \num{0.0149396516311582} & \num{2.90631103515625} & 8 & \num{0.284} & \num{-6577.426979028} & \num{0.00975772265504146} &  \num{9.12598037719727}\\ \cline{2-10}
 & 5 & \num{-6469.88864568716} & \num{0.0101865528886495} & \num{5.73368072509766} & 9 & \num{0.195333333333333} & \num{-6557.625439289} & \num{0.00671781696917542} &  \num{31.0541648864746}\\ \cline{2-10}
 & 6 & \num{-6490.41153511623} & \num{0.00704680303468339} & \num{10.2829933166504} & 9 &  &  & &\\ \cline{2-10}
 & 7 & \num{-6505.75274267646} & \num{0.00469978682318115} & \num{17.1820487976074} & 9  &  &  & &\\ \cline{2-10}
 ($3964$)& 8 & \num{-6517.1694087868} & \num{0.00295317722044436} & \num{27.1599235534668} & 9 &  &  & &\\ \cline{2-10}
 & 9 & \num{-6525.67986832392} & \num{0.00165118150579569} & \num{41.0288352966309} & 10 &  &  & &\\ \cline{2-10}
 & 10 & \num{-6532.42302989991} & \num{0.000619560658903928} & \num{59.6609878540039} & 10 &  &  & &\\ \cline{2-10}
 & 12 & \num{-6541.70623566722} & \num{0.00080065573182339} & \num{114.860893249512} & 12  &  &  & &\\ \cline{2-10}
 & fit & \num{-6536.472771} & &  & & fit & \num{-6513.866477} & &\\ \hline
 \multirow{11}{*}{1qgt} & 2 & \num{-18411.4421562182} & \num{0.024367714059874} & \num{1.22034072875977}  & 6 & \num{0.569} & \num{-19075.61262721} & \num{0.0121897934825319} &  \num{2.93578720092773} \\ \cline{2-10}
 & 3 & \num{-18603.473719048} & \num{0.0141918575991666} & \num{3.10445785522461} & 8 & \num{0.484} & \num{-19041.82811557} & \num{0.0103971203701085} &  \num{4.79096221923828}\\ \cline{2-10}
 & 4 & \num{-18701.0889144772} & \num{0.00901917555443509} & \num{6.93324279785156} & 9 & \num{0.29} & \num{-18962.98615074} & \num{0.00621360953569361} &  \num{24.803279876709}\\ \cline{2-10}
 & 5 & \num{-18757.4012897164} & \num{0.00603515230871764} & \num{13.7356567382813} & 10 & &  & &\\ \cline{2-10}
 & 6 & \num{-18793.3707075102} & \num{0.0041291133896399} & \num{24.7673568725586} & 10 & &  & &\\ \cline{2-10}
 & 7 & \num{-18819.8066359589} & \num{0.00272825923142047} & \num{41.5117835998535} & 11 & &  & &\\ \cline{2-10}
 ($9046$)& 8 & \num{-18839.1510250916} & \num{0.00170318958019394} & \num{65.6922149658203} & 11 & & & &\\ \cline{2-10}
 & 9 & \num{-18853.5883421898} & \num{0.000938148332265299} & \num{99.2851943969727} & 11 & & & &\\ \cline{2-10}
 & 10 & \num{-18864.8897524964} & \num{0.000339280482684426} & \num{144.505081176758} & 11 & & & &\\ \cline{2-10}
 & 12  & \num{-18880.1517753136} &\num{0.000469462367705731} &  \num{279.629970550537} & 11 & & & &\\ \cline{2-10}
 & fit & \num{-18871.29241} & &  & & fit & \num{-18845.88518} & &\\ \hline
\end{tabular}
\caption{Solvation energy, memory, and number of iterations for ddLPB and APBS. "Rel. En." stands for the relative energy,  "Mem." stands for the memory,  "Iter." stands for the number of macro-iterations,  and "$h$" stands for the grid spacing (APBS).}
\label{tab:sol_energy_2}
\end{table}
